A Kronecker-factored approximate Fisher matrix for convolution layers

Second-order optimization methods such as natural gradient descent have the potential to speed up training of neural networks by correcting for the curvature of the loss function. Unfortunately, the exact natural gradient is impractical to compute for large models, and most approximations either require an expensive iterative procedure or make crude approximations to the curvature. We present Kronecker Factors for Convolution (KFC), a tractable approximation to the Fisher matrix for convolutional networks based on a structured probabilistic model for the distribution over backpropagated derivatives. Similarly to the recently proposed Kronecker-Factored Approximate Curvature (K-FAC), each block of the approximate Fisher matrix decomposes as the Kronecker product of small matrices, allowing for efficient inversion. KFC captures important curvature information while still yielding comparably efficient updates to stochastic gradient descent (SGD). We show that the updates are invariant to commonly used reparameterizations, such as centering of the activations. In our experiments, approximate natural gradient descent with KFC was able to train convolutional networks several times faster than carefully tuned SGD. Furthermore, it was able to train the networks in 10-20 times fewer iterations than SGD, suggesting its potential applicability in a distributed setting.

==> discard.tex <==





\subsection{Accounting for spatial correlations}
\label{sec:spatial_correlations}

The {\bf SUD} approximation is very severe, since it ignores the spatial correlations between the pre-activation derivatives, which can be substantial in practice. Fortunately, it can be replaced with a less severe approximation that accounts for these correlations (while maintaining tractability) by approximating the pre-activation derivative covariance as factoring into a spatial term and a term for different feature maps.  This is given below:
\begin{itemize}
\item {\bf Factorized derivative correlations (FDC).} The (uncentered) covariance between any two pre-activation derivatives can be factored into a term which depends only on the feature maps and a term which depends only on spatial offset:
\begin{equation}
\autoGrad(\outputMapIdx, \outputMapIdx^\prime, \spatOffset) = \autoGradMaps(\outputMapIdx, \outputMapIdx^\prime) \autoGradSpat(\spatOffset). \label{eqn:fgc}
\end{equation}
\end{itemize}
Note that {\bf FDC} effectively amounts to assuming that the spatial correlations in derivatives are shared between different feature maps. (We investigate this approximation empirically in Section~\ref{sec:eval_assumptions}.)  Also note that {\bf FDC} is a strictly weaker assumption that {\bf SUD}, since the latter corresponds to setting $\autoGradSpat$ to a delta function at 0 in Eqn.~\ref{eqn:fgc}.

As it turns out, {\bf FDC} is enough to yield a tractable update rule:
\begin{theorem}
Combining approximations {\bf IAD}, {\bf SH}, and {\bf FDC} yields the following factorization:
\begin{equation}
\expect \left[ \gradWeightsIJS{\outputMapIdx}{\inputMapIdx}{\spatOffset} \gradWeightsIJS{\outputMapIdx^\prime}{\inputMapIdx^\prime}{\spatOffset^\prime} \right] = \numLocs \autoGradMaps(\outputMapIdx, \outputMapIdx^\prime) \autoActivationsConv(\inputMapIdx, \inputMapIdx^\prime, \spatOffset^\prime - \spatOffset), \label{eqn:full_kfc}
\end{equation}
where 
\begin{equation}
\autoActivationsConv(\inputMapIdx, \inputMapIdx^\prime, \spatOffset^\prime - \spatOffset) = \expect \left[ \activationsJS{\inputMapIdx}{\spatIdx+\spatOffset} \sum_{\spatIdx^\prime} \autoGradSpat(\spatIdx^\prime - \spatIdx) \activationsJS{\inputMapIdx^\prime}{\spatIdx^\prime+\spatOffset^\prime} \right]. \label{eqn:auto_activations_conv}
\end{equation}
\end{theorem}
\begin{proof}
See Appendix~\ref{app:proofs}.
\end{proof}
Eqn~\ref{eqn:auto_activations_conv} amounts to convolving the activations with $\autoGradSpat$ before computing their autocovariances. This results in a Kronecker factorization of the Fisher block as $\fisherMatApproxL{\layerIdx} = \convKronActConvL{\layerIdx} \otimes \convKronGradMapsL{\layerIdx}$, where $[\convKronActConvL{\layerIdx}]_{\inputMapIdx \numOffsets + \spatOffset, \inputMapIdx^\prime \numOffsets + \spatOffset^\prime} = \autoActivationsConv(\inputMapIdx, \inputMapIdx^\prime, \spatOffset^\prime - \spatOffset)$ and $[\convKronGradMapsL{\layerIdx}]_{\outputMapIdx, \outputMapIdx^\prime} = \autoGradMaps(\outputMapIdx, \outputMapIdx^\prime)$. (The $*$ subscript notation is meant to suggest that the computation requires an additional convolution operation.) The factors are exactly the same sizes as those computed in KFC-SUD, so the two Kronecker factorizations can be used interchangeably in the rest of the algorithm.

So far, we have ignored the entries of $\fisherMatL{\layerIdx}$ corresponding to bias parameters. The matrix $\convKronActConvL{\layerIdx}$ must be extended with an additional row and column to account for the bias parameters. Unfortunately, one cannot simply fold them into the weights by appending a homogeneous coordinate, as is done in the original K-FAC method (see Section~\ref{sec:kfac}). Appendix~\ref{app:biases} gives a full description of the method which accounts for the biases.





\subsection{Proof}

\setcounter{theorem}{1}
\begin{theorem}
Combining approximations {\bf IAD}, {\bf SH}, and {\bf FDC} yields the following factorization:
\begin{equation}
\expect \left[ \gradWeightsIJS{\outputMapIdx}{\inputMapIdx}{\spatOffset} \gradWeightsIJS{\outputMapIdx^\prime}{\inputMapIdx^\prime}{\spatOffset^\prime} \right] = \numLocs \autoGrad(\outputMapIdx, \outputMapIdx^\prime) \autoActivationsConv(\inputMapIdx, \inputMapIdx^\prime, \spatOffset^\prime - \spatOffset), \label{eqn:full_kfc}
\end{equation}
where 
\begin{equation}
\autoActivationsConv(\inputMapIdx, \inputMapIdx^\prime, \spatOffset^\prime - \spatOffset) = \expect \left[ \activationsJS{\inputMapIdx}{\spatIdx+\spatOffset} \sum_{\spatIdx^\prime} \autoGradSpat(\spatIdx^\prime - \spatIdx) \activationsJS{\inputMapIdx^\prime}{\spatIdx^\prime+\spatOffset^\prime} \right].
\end{equation}
\end{theorem}
\begin{proof}
We begin by restating Eqn.~\ref{eqn:iag_sh_only}, which was derived using only {\bf IAD} and {\bf SH}. We then plug in the {\bf FDC} factorization (Eqn.~\ref{eqn:fgc}) and simplify:
\begin{align}
\expect \left[ \gradWeightsIJS{\outputMapIdx}{\inputMapIdx}{\spatOffset} \gradWeightsIJS{\outputMapIdx^\prime}{\inputMapIdx^\prime}{\spatOffset^\prime} \right]
&= \sum_{\spatIdx \in \spatIdxSet} \sum_{\spatIdx^\prime \in \spatIdxSet} \expect \left[ \activationsJS{\inputMapIdx}{\spatIdx+\spatOffset} \activationsJS{\inputMapIdx^\prime}{\spatIdx^\prime+\spatOffset^\prime} \right] \expect \left[ \gradPreActivationsIS{\outputMapIdx}{\spatIdx} \gradPreActivationsIS{\outputMapIdx^\prime}{\spatIdx^\prime} \right] \\
&= \sum_{\spatIdx \in \spatIdxSet} \sum_{\spatIdx^\prime \in \spatIdxSet} \expect \left[ \activationsJS{\dimIdxTwo}{\spatIdx+\spatOffset} \activationsJS{\dimIdxTwo^\prime}{\spatIdx^\prime+\spatOffset^\prime} \right] \autoGradMaps(\outputMapIdx, \outputMapIdx^\prime) \autoGradSpat(\spatIdx^\prime - \spatIdx) \\
&= \autoGradMaps(\outputMapIdx, \outputMapIdx^\prime) \sum_{\spatIdx \in \spatIdxSet} \sum_{\spatIdx^\prime \in \spatIdxSet} \expect \left[ \activationsJS{\dimIdxTwo}{\spatIdx+\spatOffset} \activationsJS{\dimIdxTwo^\prime}{\spatIdx^\prime+\spatOffset^\prime} \right] \autoGradSpat(\spatIdx^\prime - \spatIdx) \\
&= \autoGradMaps(\outputMapIdx, \inputMapIdx) \sum_{\spatIdx \in \spatIdxSet} \expect \left[ \activationsJS{\inputMapIdx}{\spatIdx+\spatOffset} \sum_{\spatIdx^\prime \in \spatIdxSet} \autoGradSpat(\spatIdx^\prime - \spatIdx) \activationsJS{\inputMapIdx^\prime}{\spatIdx^\prime+\spatOffset^\prime} \right] \\
&= \autoGradMaps(\outputMapIdx, \outputMapIdx^\prime) \sum_{\spatIdx \in \spatIdxSet} \autoActivationsConv(\inputMapIdx, \inputMapIdx^\prime, \spatOffset^\prime - \spatOffset) \\
&= \numLocs \autoGradMaps(\outputMapIdx, \outputMapIdx^\prime) \autoActivationsConv(\inputMapIdx, \inputMapIdx^\prime, \spatOffset^\prime - \spatOffset),
\end{align}
where
\begin{equation}
\autoActivationsConv(\inputMapIdx, \inputMapIdx^\prime, \spatOffset^\prime - \spatOffset) \triangleq \expect \left[ \activationsJS{\inputMapIdx}{\spatIdx+\spatOffset} \sum_{\spatIdx^\prime} \autoGradSpat(\spatIdx^\prime - \spatIdx) \activationsJS{\inputMapIdx^\prime}{\spatIdx^\prime+\spatOffset^\prime} \right] 
\end{equation}
This yields the desired formula. In order to check that $\autoActivationsConv$ is well-defined, we need to verify that it doesn't depend on $\spatIdx$. We can do this by using our assumption {\bf SH} to write this in terms of the activation correlations and then eliminate $\spatIdx$:
\begin{align}
\autoActivationsConv(\inputMapIdx, \inputMapIdx^\prime, \spatOffset^\prime - \spatOffset) &= \sum_{\spatIdx^\prime \in \spatIdxSet} \autoGradSpat(\spatIdx^\prime - \spatIdx) \expect \left[ \activationsJS{\inputMapIdx}{\spatIdx+\spatOffset} \activationsJS{\inputMapIdx^\prime}{\spatIdx^\prime+\spatOffset^\prime} \right] \\
&= \sum_{\spatIdx^\prime \in \spatIdxSet} \autoGradSpat(\spatIdx^\prime - \spatIdx) \autoActivations(\inputMapIdx, \inputMapIdx^\prime, \spatIdx^\prime + \spatOffset^\prime - \spatIdx - \spatOffset) \\
&= \sum_r \autoGradSpat(r) \autoActivations(\inputMapIdx, \inputMapIdx^\prime, r + \spatOffset^\prime - \spatOffset).
\end{align}
\TODO{handle bounds correctly}
\end{proof}





